Search for a high-mass Higgs boson decaying to a $W$ boson pair in $pp$ collisions at $\sqrt{s} = 8$ TeV with the ATLAS detector

A search for a high-mass Higgs boson $H$ is performed in the $H\to{WW}\to\ell\nu\ell\nu$ and $H\to{WW}\to\ell\nu{qq}$ decay channels, using $pp$ collision data corresponding to an integrated luminosity of 20.3 fb$^{-1}$, collected at $\sqrt{s}=$ 8 TeV by the ATLAS detector at the Large Hadron Collider. No evidence of a high-mass Higgs boson is found. Limits on $\sigma_H\times \mathrm{BR}(H\to{WW})$ as a function of the Higgs boson mass $m_H$ are determined in three different scenarios: one in which the heavy Higgs boson has a narrow width compared to the experimental resolution, one a width increasing with the boson mass and modeled by the complex-pole scheme following the same behavior as in the Standard Model, and one for intermediate widths. The upper range of the search is $m_H=1500$ GeV for the narrow-width scenario and $m_H=1000$ GeV for the other two scenarios. The lower edge of the search range is $200-300$ GeV and depends on the analysis channel and search scenario. For each scenario, individual and combined limits from the two $WW$ decay channels are presented. At $m_H = 1500$ GeV, the highest mass point tested, $\sigma_H\cdot\mathrm{BR}(H\rightarrow WW)$ for a narrow-width Higgs boson is constrained to be less than 22 fb and 6.6 fb at the 95% CL for the gluon fusion and vector-boson fusion production modes, respectively.

==> auxmat.tex <==
\section{Auxiliary material}
\begin{figure}[bh!]
\centering
\includegraphics[width=0.48\textwidth]{fig_lvlv_mt_figure1_left_emme_ptmiss.pdf}
\includegraphics[width=0.48\textwidth]{fig_lvlv_mt_figure1_right_eemm_ptmiss.pdf}
\caption{Track-based missing transverse momentum distributions 
	 for different-flavour (left) and same-flavour (right) final states in the $\hwwlnln$ analysis, 
	   after the event preselection and before any $\MPT$ or $\METcalo$ selection.
	   The $\Njet$ categories are not separated in these figures. The histograms for the
	 background processes, including $H[125\GeV]$, are shown stacked, 
	and the distribution for a hypothetical CPS-lineshape signal process with $\mH=600\GeV$ and 
	  the cross section predicted by the SM for that mass is overlaid. 
  	 The combined statistical and systematic uncertainties on the prediction are shown by the 
	 hatched band in the upper pane and the shaded band 
	 in the lower pane.  In each figure, the last bin contains the overflow.}
\label{fig:MetPreSel} 
\end{figure}

\begin{figure}[bh!]
\centering
\includegraphics[width=0.48\textwidth]{fig_lvlv_mt_figure2_topleft_ll_mll.pdf}
\includegraphics[width=0.48\textwidth]{fig_lvlv_mt_figure2_topright_ll_mll.pdf}
\includegraphics[width=0.48\textwidth]{fig_lvlv_mt_figure2_bottom_ll_mll.pdf}
\caption{Dilepton invariant mass distributions in the 0-jet (top left), 1-jet (top
         right) and $\geq$ 2 jet (bottom) categories before applying the $\hwwlnln$ analysis selection on
	 $\mll$ and \detall. The different-flavour and same-flavour final states
	 are shown combined. The histograms for the background processes, including $H[125\GeV]$, are shown stacked, 
	and the distribution for a hypothetical CPS-lineshape signal process with $\mH=600\GeV$ and 
	  the cross section predicted by the SM for that mass is overlaid. 
	 The combined statistical and systematic uncertainties on the 
	 prediction are shown by the hatched band in the upper pane and the shaded band in the lower pane. In each figure,
	 the last bin contains the overflow.
	 }
\label{fig:MllHigh1} 
\end{figure}


